Learning Practical Communication Strategies in Cooperative Multi-Agent Reinforcement Learning

In Multi-Agent Reinforcement Learning, communication is critical to encourage cooperation among agents. Communication in realistic wireless networks can be highly unreliable due to network conditions varying with agents' mobility, and stochasticity in the transmission process. We propose a framework to learn practical communication strategies by addressing three fundamental questions: (1) When: Agents learn the timing of communication based on not only message importance but also wireless channel conditions. (2) What: Agents augment message contents with wireless network measurements to better select the game and communication actions. (3) How: Agents use a novel neural message encoder to preserve all information from received messages, regardless of the number and order of messages. Simulating standard benchmarks under realistic wireless network settings, we show significant improvements in game performance, convergence speed and communication efficiency compared with state-of-the-art.

==> 2_background.tex <==
\section{Background}
\label{sec: background}

\subsection{Reinforcement Learning}
\label{sec: background rl}

Reinforcement learning (RL) teaches an agent how to intelligently act in an environment, in order to maximize some long-term, cumulative reward. 
In an RL problem, there are four major events: 
making an \emph{observation}, taking an \emph{action}, transitioning to a new \emph{state} and receiving a \emph{reward}. 
Denote $o$ as the observation, and so the observation space, $\mathcal{O}$, is the set consisting of all possible $o$. 
Similarly, denote $a$ as the action $\mathcal{A}$ as the action space; $s$ as the state and $\mathcal{S}$ as the state space. Denote the scalar $r$ as the reward value.
We further define \emph{policy} $\pi$ as a strategy to select an action from a state. 
\ie, $\pi: \mathcal{S}\rightarrow \mathcal{A}$. 
The policy can be either deterministic or stochastic. For stochastic $\pi$, the mapping to $\mathcal{A}$ follows a probability distribution. 
We can thus more formally describe the RL problem: 
at time step $t$, the agent is in state $s_t\in\mathcal{S}$. It observes $o_t\in\mathcal{O}$ from the environment, takes an action $a_t\in\mathcal{A}$ according to policy $\pi\paren{\cdot |s_t}$, receives reward $r_t$ from the environment and transits to state $s_{t+1}$. 

Our goal is to find an optimum policy $\pi^*$ that maximizes the expected long-term reward (\ie, return) $J = \mathbb{E}_{\pi}\left[\sum_{t=1}^{\infty}\gamma^{t} r_t\right]$, where $\gamma\in [0,1]$ is called the discount factor.

\subsubsection{Challenges}

In practice, the state space and action space are huge, and thus it may take the agent enormous exploration in the environment to identify a good policy. 
Unfortunately the interaction with the environment can often be very expensive and time-consuming. So various techniques are necessary to help speedup the convergence to a good $\pi$. 
The first way is to combine deep learning techniques with RL, by taking advantage of DNN's ability as universal function approximators \citep{universal}. 
Going back to the calculation of the return $J$, we note that $J$ involves $r_{t'}$ of future steps (\ie, $t'>t$). 
So to estimate $J$, a common way is to treat $J$ as a function $R\paren{s_t, a_t, s_{t+1}}$. Then we can train a DNN to approximate $R$ where only data of the current transition are required. 
Due to the generalization capability of DNNs, such a design can efficiently learn $\pi$ from limited amount of training data. 
The second way is by carefully defining (or, re-defining) the observation space $\mathcal{O}$ so that the agent can have better or richer information about the dynamics of the environment. 
An example is training agents to play the StarCraft game. In \cite{smac}, if we allow the agent to observe its allies past few actions, the training will learn a much better policy. 
In our work, we augment $\mathcal{O}$ by wireless network observations to improve agents' policy (see Section \ref{sec: method what}). 
The third way is to modify the training algorithm to allow reuse of data from previous environment interactions, which we discuss next. 

\subsubsection{On-Policy \emph{vs.} Off-Policy}
RL algorithms can be classified as on-policy and off-policy. 
Denote $\theta$ as the model parameters for the policy, and thus we denote policy as $\pi_\theta$. 
In the training process, $\theta$ keeps getting updated, and thus agent's interactions with the environment are corrected under constantly evolving policies $\pi_\theta$. 
For on-policy algorithms, every policy update is only based on data collected from the current (\ie, most recent) $\pi_\theta$. So when $\theta$ is updated to $\theta'$, the data collected from $\pi_{\theta}$ are discarded. 
For off-policy algorithms, the data collected from previous policies can be reused to updated the correct policy. 
Such historical data may be stored in an experience replay buffer \citep{experience_replay} to facilitate reuse. 
Therefore, there are trade-offs between the two types. On-policy algorithms may be more stable and easier to tune, while off-policy ones are more sample efficient \citep{p3o}. 
In general, both on-policy and off-policy algorithms can be useful, depending on the application. 
Our proposed framework can improve the performance of both (Sections \ref{sec: method generalize marl}, \ref{sec: exp}). 



\subsection{Multi-Agent Reinforcement Learning}
\label{sec: background marl}

When extending RL algorithms to multiple agents, the following challenges emerge. 
Firstly, the action and state space becomes significantly larger -- exponential with the number of agents. 
Secondly, the environment becomes non-stationary \citep{nonstationary} since all agents are updating their policies simultaneously. 
Thirdly, there can be three types of agent relationships: cooperative, competitive and mixed \citep{ic3net, marl_overview}. 
Depending on the relationship, the algorithm can learn significantly different policies. 
In this paper, we focus on cooperative agents, where all agents share a common goal. 
Finally, the MARL environment is partially observable. \ie, each agent does not see the full status of the environment or the state / action of the other agents. 

To address the challenges, communication among agents is important. 
The extra information conveyed by agents' messages guide agents to better explore the huge state and action space, and thus may improve convergence speed and quality. 
The information sharing may also promote collaboration and alleviate the limitation of partial observability. 
In the search-and-rescue (SAR) example, each robot can only sense a small region around it, without seeing the full terrain. 
Sharing the local terrain observations may lead to better route planning and thus shorter time to rescue the target. 

In this paper, the key issue we aim at addressing is how to make communication among agents intelligent. 
We improve from the three fundamental aspects of communication (\ie, ``when'', ``what'' and ``how'') so that we fully exploit the benefits of communication in MARL. 


\subsection{Communication Among Agents}
\label{sec: background comm}

With the wireless network environment, even if an agent decides to send a message, it is not guaranteed that the other agents can successfully receive the message. 
Possible reasons for not receiving a message include path loss, fading and contention.
A path loss model with log-normal fading is widely used to capture the Radio Signal Strength (RSS) variation over the spatial domain (see Appendix ??.? for details).
Agents also contend to access the medium. For example, in $p$-CSMA, agents sense and contend with probability $p$. 
Interference can happen when the receiver is in range of multiple senders at the same time.
The signal-to-interference-plus-noise ratio (SINR) is the power ratio of received signal strength over noise and interference.
When SINR is below a threshold $\theta$, the packet cannot be decoded correctly.


==> tables/sota_comm.tex <==
\begin{tabular}{lcccc}
    \toprule
     & Method & Succ. Comm. & Total Comm. & Efficiency\\
    \midrule
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\ppw{5}}} 
        & CommNet       & 0.00\std{0.00} & 0.00\std{0.00} & 0.00\std{0.00} \\
        & IC3Net        & 0.00\std{0.00} & 0.00\std{0.00} & 0.00\std{0.00} \\
        & \proposedre   & \textbf{0.00}\std{0.00} & \textbf{0.00}\std{0.00} & \textbf{0.00}\std{0.00} \\
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\ppw{10}}} 
        & CommNet       & 0.00\std{0.00} & 0.00\std{0.00} & 0.00\std{0.00} \\
        & IC3Net        & 0.00\std{0.00} & 0.00\std{0.00} & 0.00\std{0.00} \\
        & \proposedre   & \textbf{0.00}\std{0.00} & \textbf{0.00}\std{0.00} & \textbf{0.00}\std{0.00} \\
    \bottomrule
\end{tabular}

